New Encoders for German Trained from Scratch: Comparing ModernGBERT with Converted LLM2Vec Models

Encoders remain essential for efficient German NLP and NLU scenarios despite the rise of decoder-only LLMs. This work studies two routes to high-quality German encoders under identical data and training constraints: 1) training from scratch and 2) converting decoders via LLM2Vec. We introduce two resources: ModernGBERT (134M, 1B), fully transparent German encoders in the ModernBERT style, and LL\"aMmleinVec (120M, 1B, 7B), decoder-to-encoder conversions trained with masked next-token prediction, both undergoing a context extension to 8.192 tokens. Across SuperGLEBer, ModernGBERT 1B sets a new state of the art (avg 0.808), surpassing GBERT Large (+4%) and the seven-times larger converted 7B model (0.787). On German MTEB after supervised fine-tuning, ModernGBERT 1B (0.551) approaches the converted 7B model (0.557). We release all models, checkpoints, datasets, and full training records, and introduce an encoder-adapted QA-NIAH evaluation. All in all, our results provide actionable guidance: when parameter efficiency and latency matter, from-scratch encoders dominate. When a pre-trained decoder exists and compute is a limited, conversion offers an effective alternative. ModernGBERT and LL\"aMmleinVec, including all code, data and intermediary checkpoints are published under a research-only RAIL license.

==> details_table_llm2vec.tex <==

\begin{table*}[!t]
    \small
    \centering
    \begin{tabular}{lcccccc} % Adjusts to content width
        \toprule
                            & \multicolumn{2}{c}{\LLaMmleinVec 120M} & \multicolumn{2}{c}{\clap{\LLaMmleinVec 1B}} & \multicolumn{2}{c}{\clap{\LLaMmleinVec 7B}}                                                                                                             \\
        \cmidrule{2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
                            & Ext1                                   & Ext2                                        & {\hbox to 1.8cm{\hfil Ext1\hfil}}           & {\hbox to 1.8cm{\hfil Ext2\hfil}} & {\hbox to 1.8cm{\hfil Ext1\hfil}} & {\hbox to 1.8cm{\hfil Ext2\hfil}} \\
        \midrule
        Training Tokens     & 52B                                    & 14.4B                                       & 90B                                         & 14.4B                             & 90B                               & 14.4B                             \\
        Max Sequence Length & \multicolumn{2}{c}{\num{8192}}         & \multicolumn{2}{c}{\num{8192}}              & \multicolumn{2}{c}{\num{8192}}                                                                                                                          \\
        RoPE theta          & \multicolumn{2}{c}{\num{160000}}       & \multicolumn{2}{c}{\num{160000}}            & \multicolumn{2}{c}{\num{160000}}                                                                                                                        \\

        \midrule
        Batch Size          & 32                                     & 32                                          & 32                                          & 32                                & 16                                & 16                                \\
        \midrule
        Training Hardware   & \multicolumn{2}{c}{64$\times$ H200}    & \multicolumn{2}{c}{64$\times$ H200}         & 256  $\times$ H200                          & 128    $\times$ H200                                                                                      \\
        Training Duration   & 10h41                                  & 3h40                                        & 37h24                                       & 6h40                              & 14h25${}^\dagger$                 & 9h39                              \\
        \bottomrule
    \end{tabular}
    \caption{\LLaMmleinVec training settings. Due to limited resources we had to terminate the 7B model training on the first extension dataset early ${}^\dagger$.}
    \label{tab:llm2vec-training}
\end{table*}


==> details_tables_moderngbert.tex <==

\begin{table*}[!t]
    \small
    \centering
    \begin{tabular}{lcccccc} % Adjusts to content width
        \toprule
                                    & \multicolumn{2}{c}{Pretraining Phase}                                & \multicolumn{2}{c}{\clap{Context Extension: Phase One}} & \multicolumn{2}{c}{\clap{Context Extension: Phase Two}}                                                                                                         \\
        \cmidrule{2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
                                    & 134M                                                                 & 1B                                                      & {\hbox to 1.8cm{\hfil 134M\hfil}}                       & {\hbox to 1.8cm{\hfil 1B\hfil}} & {\hbox to 1.8cm{\hfil 134M\hfil}} & {\hbox to 1.8cm{\hfil 1B\hfil}} \\
        \midrule
        Training Tokens             & 0.47T                                                                & 1.27T                                                   & 52B                                                     & 90B                             & \multicolumn{2}{c}{14.4B}                                           \\
        Max Sequence Length         & \multicolumn{2}{c}{\num{1024}}                                       & \multicolumn{2}{c}{\num{8192}}                          & \multicolumn{2}{c}{\num{8192}}                                                                                                                                  \\
        RoPE Theta                  & \multicolumn{2}{c}{\num{10000}}                                      & \multicolumn{2}{c}{\num{160000}}                        & \multicolumn{2}{c}{\num{160000}}                                                                                                                                \\
        \midrule
        Batch Size                  & \num{4608}                                                           & \num{4928}                                              & 96                                                      & 96                              & 96                                & 96                              \\
        \hspace{3mm}Warmup (tokens) & \multicolumn{2}{c}{\num{3e9}}                                        & ---                                                     & ---                                                     & ---                             & ---                                                                 \\
        Microbatch Size             & 96                                                                   & 28                                                      & 8                                                       & 3                               & 8                                 & 3                               \\
        \midrule
        Learning Rate               & \num{8e-4}                                                           & \num{5e-5}                                              & \num{3e-4}                                              & \num{5e-5}                      & \num{3e-4}                        & \num{5e-6}                      \\
        \hspace{3mm}Schedule        & \multicolumn{2}{c}{Trapezoidal}                                      & ---                                                     & ---                                                     & \multicolumn{2}{c}{1-sqrt}                                                                            \\
        \hspace{3mm}Warmup (tokens) & \multicolumn{2}{c}{\num{15e9}}                                       & ---                                                     & ---                                                     & ---                             & ---                                                                 \\
        \hspace{3mm}Decay (tokens)  & ---                                                                  & ---                                                     & ---                                                     & ---                             & \multicolumn{2}{c}{\num{12.8e9}}                                    \\
        Weight Decay                & \multicolumn{2}{c}{\num{1e-5}}                                       & \num{1e-5}                                              & \num{1e-6}                                              & \num{1e-5}                      & \num{1e-6}                                                          \\
        \midrule
        Training Time (hours)       & \num{31.3}                                                           & \num{446.1}                                             & \num{5.9}                                               & \num{42.1}                      & \num{2.0}                         & \num{8.3}                       \\
        \midrule
        Model Initialization        & Megatron                                                             & Megatron                                                & ---                                                     & ---                             & ---                               & ---                             \\
        \midrule
        Dropout (attn out)          & \multicolumn{6}{l}{\hspace{1.2mm}0.1}                                                                                                                                                                                                                                                            \\
        Dropout (all other layers)  & \multicolumn{6}{l}{\hspace{1.2mm}0.0}                                                                                                                                                                                                                                                            \\
        \midrule
        Optimizer                   & \multicolumn{6}{l}{\hspace{1.2mm}StableAdamW}                                                                                                                                                                                                                                                    \\
        \hspace{1.2mm}Betas         & \multicolumn{6}{l}{\hspace{1.2mm}(0.90, 0.98)}                                                                                                                                                                                                                                                   \\
        \hspace{1.2mm}Epsilon       & \multicolumn{6}{l}{\hspace{1.2mm}\num{1e-06}}                                                                                                                                                                                                                                                    \\
        \midrule
        Training Hardware           & \multicolumn{6}{l}{\hspace{1.2mm}16$\times$ H100}                                                                                                                                                                                                                                                \\
        Training Strategy           & \multicolumn{6}{l}{\hspace{1.2mm}Distributed DataParallel, bfloat16}                                                                                                                                                                                                                             \\
        %Software Libraries          & \multicolumn{6}{l}{\hspace{1.2mm}PyTorch 2.3.0, Cuda 12.8.0, Composer 0.22.0, Flash Attention 2.6.3, FA3 commit bc482cb}                                                                                                                                                                                                                             \\
        \bottomrule
    \end{tabular}
    \caption{\modernGBERT training settings. Dropout and below are shared across all phases.}
    \label{tab:modernbert-training}
\end{table*}


==> result_table_niah.tex <==
\begin{table*}
        \centering
        \small\begin{tabular}{l@{}r|ccc||c}
                \toprule
                {Model}                          & {Params} &
                {\makecell[b]{\num{<1024} tok.}} &
                {\makecell[b]{\num{1024} to                                                                                       \\\num{4095} tok.}} &
                {\makecell[b]{\num{4096} to                                                                                       \\\num{8192} tok.}} & {Overall}\\
                \midrule
                \LLaMmlein                       & 120M     & 0.286           & 0.124           & 0.049          & 0.091          \\
                \LLaMmlein                       & 1B       & 0.517           & 0.230           & 0.088          & 0.165          \\
                \LLaMmlein                       & 7B       & 0.529           & 0.310           & 0.122          & 0.216          \\
                \midrule
                \LLaMmleinVec (ext1)             & 120M     & 0.315           & 0.206           & 0.044          & 0.120          \\
                \LLaMmleinVec (ext2)             & 120M     & 0.252           & 0.047           & 0.000          & 0.031          \\
                \LLaMmleinVec (ext1+2)           & 120M     & 0.055           & 0.001           & 0.000          & 0.003          \\[1ex]
                \LLaMmleinVec (ext1)             & 1B       & 0.588           & 0.448           & 0.232          & 0.333          \\
                \LLaMmleinVec (ext2)             & 1B       & 0.555           & 0.297           & 0.003          & 0.144          \\
                \LLaMmleinVec (ext1+2)           & 1B       & 0.462           & 0.209           & 0.033          & 0.123          \\[1ex]
                \LLaMmleinVec (ext1)             & 7B       & 0.597           & 0.207           & 0.000          & 0.111          \\
                \LLaMmleinVec (ext2)             & 7B       & 0.605           & 0.176           & 0.000          & 0.099          \\
                \LLaMmleinVec (ext1+2)           & 7B       & 0.580           & 0.327           & 0.000          & 0.156          \\
                \midrule
                \modernGBERT                     & 134M     & 0.552           & 0.168           & 0.013          & 0.105          \\
                \modernGBERT + ext1              & 134M     & 0.536           & 0.410           & 0.238          & 0.323          \\
                \modernGBERT + ext1+2            & 134M     & 0.540           & 0.393           & 0.201          & 0.296          \\[1ex]
                \modernGBERT                     & 1B       & 0.556           & 0.233           & 0.023          & 0.136          \\
                \modernGBERT+ ext1               & 1B       & \bfseries 0.617 & 0.506           & \textbf{0.406} & \textbf{0.457} \\
                \modernGBERT  + ext1+2           & 1B       & 0.601           & \bfseries 0.526 & 0.383          & 0.451          \\
                \bottomrule
        \end{tabular}
        \caption{QA-NIAH results. Metric is Exact Match. All tokens are counted per the model's respective tokenizer.
                \modernGBERT models marked with ``w/o ext'' refer to the model checkpoint after pre-training but before the context extension phases, those marked with ``w/o ext2'' to the models after extension phase one, but before phase two.}\label{tab:niah}
\end{table*}


==> result_table_supergleber.tex <==
\begin{sidewaystable*}
   \centering\small
   \begin{tabular}{ll@{}rl|ccccc|c||cc|c||c||c||c}
      \toprule
                                           &                                                                &        &                &
      \multicolumn{6}{c||}{classification} &
      \multicolumn{3}{c||}{tagging}        & \multirow{4}{*}{\rotatebox[origin=c]{270}{\makecell{similarity                                                                                                                                                                                                                              \\pearson corr}}}                               & \multirow{4}{*}{\rotatebox[origin=c]{270}{\makecell{QA                                                                                                                                                                       \\m.\ t.\ F1}}} & \multirow{4}{*}{\rotatebox[origin=c]{270}{\makecell{Average                                                                                                                                                                       \\mixed}}}                                                                                                                                                                                \\
      type                                 & model                                                          & params &                &
      \rotatebox[origin=c]{270}{\makecell{tox.                                                                                                                                                                                                                                                                                           \\macro F1}}     &
      \rotatebox[origin=c]{270}{\makecell{sent.                                                                                                                                                                                                                                                                                          \\micro F1}}            &
      \rotatebox[origin=c]{270}{\makecell{match                                                                                                                                                                                                                                                                                          \\ACC}}                 &
      \rotatebox[origin=c]{270}{\makecell{WSD                                                                                                                                                                                                                                                                                            \\micro F1}}              &
      \rotatebox[origin=c]{270}{\makecell{other                                                                                                                                                                                                                                                                                          \\mixed}}                     &
      \rotatebox[origin=c]{270}{\makecell{avg                                                                                                                                                                                                                                                                                            \\mixed}}                       &
      \rotatebox[origin=c]{270}{\makecell{NER                                                                                                                                                                                                                                                                                            \\micro F1}}                       &
      \rotatebox[origin=c]{270}{\makecell{other                                                                                                                                                                                                                                                                                          \\micro F1}}                     &
      \rotatebox[origin=c]{270}{\makecell{avg                                                                                                                                                                                                                                                                                            \\micro F1}}                       & &
      %\rotatebox[origin=c]{270}{embd}                      &
      %\rotatebox[origin=c]{270}{QA}
      \\ \midrule[.75pt]
      %                                                       & majority                                                      & -                                                                                                                     \\
      %                                                       & random                                                        & -                                                                                                                     \\ \midrule[.75pt]
      enc                                  &
      \GbertBASE                           & 111M                                                           &
                                           & 0.537                                                          & 0.620  & 0.738          & 0.814          & 0.749          & 0.723
                                           & 0.705                                                          & 0.806  & 0.786
                                           & 0.561                                                          & 0.803  & 0.718                                                                                                                                                                                                             \\
      enc                                  &
      \GbertLARGE                          & 337M                                                           &
                                           & 0.604                                                          & 0.673  & 0.810          & 0.837          & 0.816          & 0.785
                                           & 0.744                                                          & 0.813  & 0.799
                                           & 0.654                                                          & 0.832  & 0.768                                                                                                                                                                                                             \\[1ex]


      enc                                  & gerturax-3                                                     & 135M   &                & 0.561          & 0.617          & 0.788          & 0.804          & 0.762          & 0.736          & 0.707          & 0.810          & 0.789          & 0.603          & 0.832          & 0.740 \\[1ex]


      enc                                  & \GebertaBASE ${}^\dagger$                                      & 139M   &                & 0.530          & 0.619          & 0.766          & 0.789          & 0.737          & 0.715          & 0.687          & 0.801          & 0.778          & 0.559          & 0.813          & 0.716 \\
      enc                                  & \GebertaLARGE${}^\dagger$                                      & 406M   &                & 0.551          & 0.623          & 0.783          & 0.795          & 0.775          & 0.743          & 0.736          & 0.804          & 0.791          & 0.619          & 0.844          & 0.749 \\
      enc                                  & \GebertaXLARGE${}^\dagger$                                     & 887M   &                & 0.606          & 0.671          & 0.796          & 0.830          & 0.795          & 0.770          & 0.763          & 0.818          & 0.807          & 0.643          & 0.848          & 0.767 \\[1ex]
      enc                                  & \XLMRobertaBASE                                                & 279M   &                & 0.530          & 0.546          & 0.741          & 0.790          & 0.717          & 0.693          & 0.648          & 0.780          & 0.754          & 0.505          & 0.802          & 0.689 \\


      enc                                  & \XLMRobertaLARGE                                               & 561M   &                & 0.512          & 0.559          & 0.795          & 0.814          & 0.739          & 0.714          & 0.720          & 0.804          & 0.787          & 0.583          & 0.837          & 0.730 \\
      enc                                  & \XLMRobertaXLARGE                                              & 3.48B  &                & 0.558          & 0.612          & 0.815          & 0.820          & 0.778          & 0.750          & 0.746          & 0.816          & 0.802          & 0.656          & 0.822          & 0.758 \\


      %enc      &
      %gerturax-3  & &  0.561 & 0.617 & 0.788 & 0.804 & 0.762 & 0.736 & 0.707 & 0.810 & 0.789 & 0.603 & 0.832 & 0.740  \\
      %dec & leo-hessianai-7b &  & 0.617  & 0.739   & 0.825 & 0.868  & 0.835 & 0.809 & 0.745  & 0.787 & 0.779 & 0.578 & 0.867                           \\
      \midrule
      dec                                  & Llama 3.2                                                      & 1B     &                & 0.519          & 0.629          & 0.768          & 0.808          & 0.768          & 0.737          & 0.648          & 0.733          & 0.716          & 0.551          & 0.835          & 0.710 \\

      %enc                                  & Llama2Vec 3.2                                                  & 1B     &       & 0.527 & 0.637 & 0.772 & 0.797 & 0.768 & 0.737 & 0.725 & 0.787 & 0.774 & 0.636 & 0.848 & 0.749 \\
      dec                                  & Llama 3.1                                                      & 8B     &                & 0.586          & 0.713          & 0.819          & 0.849          & 0.817          & 0.790          & 0.708          & 0.753          & 0.744          & 0.573          & 0.868          & 0.744 \\

      %enc                                  & Llama2Vec 3.1                                                  & 8B     &       & 0.595 & 0.732 & 0.809 & 0.831 & 0.823 & 0.793 & 0.782 & 0.826 & 0.817 & 0.696 & 0.885 & 0.798 \\

      \midrule

               enc &           \mmBERTSmall & 142M &  & 0.546  & 0.641 & 0.777 & 0.843 & 0.791 & 0.759 & 0.766 & 0.809 & 0.800 & 0.606 & 0.828 & 0.748 \\

         enc &        \mmBERTBase & 309M &  & 0.543  & 0.667 & 0.793 & 0.851 & 0.782 & 0.757 & 0.786 & 0.809 & 0.804 & 0.622 & 0.849 & 0.758 \\[1ex]
                  enc &           \euroBERTsmall & 212M &  & 0.418  & 0.491 & 0.738 & 0.766 & 0.691 & 0.659 & 0.550 & 0.734 & 0.698 & 0.607 & 0.859 & 0.706 \\
                    enc &         \euroBERTmid & 609M &  & 0.434  & 0.479 & 0.753 & 0.777 & 0.646 & 0.633 & 0.677 & 0.768 & 0.750 & 0.633 & 0.869 & 0.721 \\
                   enc &          \euroBERTlarge & 2.11B &  & 0.444  & 0.456 & 0.718 & 0.772 & 0.652 & 0.633 & 0.681 & 0.785 & 0.764 & 0.655 & 0.873 & 0.731 \\

      \bottomrule
   \end{tabular}
   \caption{SuperGLEBer results, averaged at varying levels of granularity, following \cite{pfister-hotho-2024-supergleber}. The columns reading “Average” have been averaged across the averages of the respective task types, in order to not overweight any task type for which more  datasets exist. ${}^\dagger$ indicates that these models were evaluated without fp16. \modernGBERT models marked with ``w/o ext.'' refer to the model checkpoint after pre-training but before the context extension phases. We also exemplary evaluated LLM2Vec after 20\% of LONG Head or Head/Middle training data (“+ 1/5 ext1“).  }
   \label{tab:subergleber}
\end{sidewaystable*}


\begin{sidewaystable*}
   \centering\small
   \begin{tabular}{ll@{}rl|ccccc|c||cc|c||c||c||c}
      \toprule
                                           &                                                                &        &                &
      \multicolumn{6}{c||}{classification} &
      \multicolumn{3}{c||}{tagging}        & \multirow{4}{*}{\rotatebox[origin=c]{270}{\makecell{similarity                                                                                                                                                                                                                              \\pearson corr}}}                               & \multirow{4}{*}{\rotatebox[origin=c]{270}{\makecell{QA                                                                                                                                                                       \\m.\ t.\ F1}}} & \multirow{4}{*}{\rotatebox[origin=c]{270}{\makecell{Average                                                                                                                                                                       \\mixed}}}                                                                                                                                                                                \\
      type                                 & model                                                          & params &                &
      \rotatebox[origin=c]{270}{\makecell{tox.                                                                                                                                                                                                                                                                                           \\macro F1}}     &
      \rotatebox[origin=c]{270}{\makecell{sent.                                                                                                                                                                                                                                                                                          \\micro F1}}            &
      \rotatebox[origin=c]{270}{\makecell{match                                                                                                                                                                                                                                                                                          \\ACC}}                 &
      \rotatebox[origin=c]{270}{\makecell{WSD                                                                                                                                                                                                                                                                                            \\micro F1}}              &
      \rotatebox[origin=c]{270}{\makecell{other                                                                                                                                                                                                                                                                                          \\mixed}}                     &
      \rotatebox[origin=c]{270}{\makecell{avg                                                                                                                                                                                                                                                                                            \\mixed}}                       &
      \rotatebox[origin=c]{270}{\makecell{NER                                                                                                                                                                                                                                                                                            \\micro F1}}                       &
      \rotatebox[origin=c]{270}{\makecell{other                                                                                                                                                                                                                                                                                          \\micro F1}}                     &
      \rotatebox[origin=c]{270}{\makecell{avg                                                                                                                                                                                                                                                                                            \\micro F1}}                       & &
      %\rotatebox[origin=c]{270}{embd}                      &
      %\rotatebox[origin=c]{270}{QA}
      \\ \midrule[.75pt]
    
      dec                                  &
      \LLaMmlein                           & 120M                                                           &
                                           & 0.510                                                          & 0.580  & 0.710          & 0.798          & 0.732          & 0.702          & 0.613          & 0.737          & 0.712          & 0.477          & 0.812          & 0.676                                                    \\
      %enc                                  &
      %LLäMmlein2Vec                        & 120M                                                           &        & 0.518 & 0.562 & 0.586 & 0.736 & 0.722 & 0.678 & 0.624 & 0.753 & 0.727 & 0.518 & 0.819 & 0.685         \\
      enc                                  &
      \LLaMmleinVec (1/5 ext1)             & 120M                                                           &        & 0.480          & 0.571          & 0.696          & 0.793          & 0.738          & 0.700          & 0.627          & 0.754          & 0.729          & 0.471          & 0.821          & 0.680                  \\

      enc                                  &
      \LLaMmleinVec (ext1)                 & 120M                                                           &        & 0.491          & 0.564          & 0.711          & 0.797          & 0.739          & 0.703          & 0.660          & 0.761          & 0.741          & 0.472          & 0.819          & 0.684                  \\
      enc                                  &
      \LLaMmleinVec (ext2)                 & 120M                                                           &        & 0.471          & 0.568          & 0.686          & 0.772          & 0.739          & 0.697          & 0.620          & 0.757          & 0.730          & 0.455          & 0.818          & 0.675                  \\
      enc                                  &
      \LLaMmleinVec (ext1+2)               & 120M                                                           &        & 0.448          & 0.490          & 0.581          & 0.749          & 0.708          & 0.657          & 0.505          & 0.728          & 0.683          & 0.439          & 0.730          & 0.627                  \\[1ex]
      %\hdashline

      dec                                  &
      \LLaMmlein                           & 1B                                                             &
                                           & 0.603                                                          & 0.710  & 0.790          & 0.839          & 0.806          & 0.781          & 0.728          & 0.785          & 0.773          & 0.548          & 0.828          & 0.733                                                    \\
      % enc                                  &
      % LLäMmlein2Vec                        & 1B                                                             &        & 0.604 & 0.703 & 0.784 & 0.835 & 0.811 & 0.782 & 0.775 & 0.818 & 0.809 & 0.631 & 0.831 & 0.763         \\
      enc                                  &
      \LLaMmleinVec (1/5 ext1)             & 1B                                                             &        & 0.587          & 0.694          & 0.827          & 0.820          & 0.806          & 0.779          & 0.795          & 0.815          & 0.811          & 0.615          & 0.842          & 0.762                  \\

      enc                                  &
      \LLaMmleinVec (ext1)                 & 1B                                                             &        & 0.575          & 0.702          & 0.775          & 0.835          & 0.808          & 0.776          & 0.790          & 0.818          & 0.812          & 0.615          & 0.843          & 0.762                  \\
      enc                                  &
      \LLaMmleinVec (ext2)                 & 1B                                                             &        & 0.528          & 0.688          & 0.754          & 0.815          & 0.789          & 0.755          & 0.775          & 0.812          & 0.804          & 0.580          & 0.836          & 0.744                  \\
      enc                                  &
      \LLaMmleinVec (ext1+2)               & 1B                                                             &        & 0.503          & 0.566          & 0.692          & 0.787          & 0.732          & 0.697          & 0.727          & 0.799          & 0.784          & 0.557          & 0.828          & 0.717                  \\[1ex]
      %\hdashline

      dec                                  &
      \LLaMmlein                           & 7B                                                             &        & 0.632          & 0.739          & 0.821          & 0.873          & 0.835          & 0.810          & 0.796          & 0.808          & 0.805          & 0.524          & 0.851          & 0.747                  \\
      %  enc                                  &
      % OLD LLäMmlein2Vec                        & 7B                                                             &        & 0.636 & 0.748 & 0.820 & 0.860 & 0.835 & 0.810 & 0.851 & 0.836 & 0.839 & 0.656 & 0.872 & 0.794         \\

      enc                                  &
      \LLaMmleinVec  (ext1)                & 7B                                                             &        & 0.633          & 0.742          & 0.813          & 0.839          & 0.822          & 0.799          & 0.851          & 0.835          & 0.838          & \textbf{0.670} & 0.842          & 0.787                  \\
      enc                                  &
      \LLaMmleinVec (ext2)                 & 7B                                                             &        & 0.612          & 0.743          & 0.808          & 0.848          & 0.822          & 0.797          & 0.848          & 0.834          & 0.837          & 0.657          & 0.842          & 0.783                  \\
      enc                                  &
      \LLaMmleinVec (ext1+2)               & 7B                                                             &        & 0.554          & 0.647          & 0.610          & 0.786          & 0.744          & 0.709          & 0.747          & 0.804          & 0.793          & 0.639          & 0.821          & 0.740                  \\
      \midrule
      enc                                  &
      \modernGBERT                         & 134M                                                           &        & 0.503          & 0.617          & 0.769          & 0.780          & 0.744          & 0.716          & 0.734          & 0.794          & 0.782          & 0.589          & 0.833          & 0.730                  \\
      enc                                  &
      \modernGBERT   + ext1+2              & 134M                                                           &        & 0.526          & 0.647          & 0.779          & 0.806          & 0.760          & 0.735          & 0.791          & 0.809          & 0.805          & 0.621          & 0.836          & 0.749                  \\[1ex]
      enc                                  &
      \modernGBERT                         & 1B                                                             &        & 0.610          & \textbf{0.746} & \textbf{0.827} & 0.858          & 0.833          & 0.806          & 0.849          & 0.837          & 0.839          & 0.681          & 0.874          & 0.800                  \\
      enc                                  &
      \modernGBERT + ext1+2                & 1B                                                             &        & \textbf{0.635} & 0.745          & 0.826          & \textbf{0.876} & \textbf{0.836} & \textbf{0.812} & \textbf{0.868} & \textbf{0.840} & \textbf{0.845} & 0.699          & \textbf{0.876} & \textbf{0.808}         \\
      \bottomrule
   \end{tabular}
   \caption{SuperGLEBer results, averaged at varying levels of granularity, following \cite{pfister-hotho-2024-supergleber}. The columns reading “Average” have been averaged across the averages of the respective task types, in order to not overweight any task type for which more  datasets exist. ${}^\dagger$ indicates that these models were evaluated without fp16. \modernGBERT models marked with ``w/o ext.'' refer to the model checkpoint after pre-training but before the context extension phases. We also exemplary evaluated LLM2Vec after 20\% of LONG Head or Head/Middle training data (“+ 1/5 ext1“).  }
   \label{tab:subergleber}
\end{sidewaystable*}


==> results_table_efficiency.tex <==
\begin{table*}
   \small
   \centering
   \begin{tabular}{l@{} r S[table-format=3.2(2),separate-uncertainty] S[table-format=3.2(2),separate-uncertainty] S[table-format=3.2(2),separate-uncertainty] S[table-format=3.2(2),separate-uncertainty]}
      \toprule
                                    &        & \multicolumn{2}{c}{Short} & \multicolumn{2}{c}{\clap{Long}}                                       \\
      \cmidrule(lr){3-4} \cmidrule(lr){5-6}
      Model                         & Params & {Fixed Length}            & {Variable Length}               & {Fixed Length}  & {Variable Length} \\
      \midrule
      \GbertBASE                    & 111M   & 2.33+-0.13                & 5.25+-0.27                      & {--}            & {--}              \\
      \GbertLARGE                   & 337M   & 7.25+-0.77                & 15.70+-1.66                     & {--}            & {--}              \\[1ex]
      gerturax-3                    & 135M   & 4.13+-0.40                & 8.26+-0.81                      & {--}            & {--}              \\[1ex]
      \GebertaBASE${}^\dagger$      & 139M   & 9.79 \pm 0.04             & 19.40 \pm 0.08                  & {--}            & {--}              \\
      \GebertaLARGE${}^\dagger$     & 406M   & 27.30 \pm 0.09            & 54.10 \pm 0.40                  & {--}            & {--}              \\
      \GebertaXLARGE${}^\dagger$    & 887M   & 42.20 \pm 0.36            & 83.80 \pm 0.70                  & {--}            & {--}              \\[1ex]
      \XLMRobertaBASE               & 279M   & 2.28\pm 0.08              & 5.05\pm 0.19                    & {--}            & {--}              \\
      \XLMRobertaLARGE${}^\dagger$  & 561M   & 7.27 \pm 0.53             & 15.90 \pm 1.04                  & {--}            & {--}              \\
      \XLMRobertaXLARGE${}^\dagger$ & 3.48B  & 57.70 \pm 0.37            & 123.00 \pm 0.71                 & {--}            & {--}              \\
      \midrule
      \LLaMmleinVec                 & 120M   & 3.74 \pm 0.75             & 7.17 \pm 0.53                   & 6.69 \pm 0.14   & 8.39 \pm 0.35     \\
      \LLaMmleinVec                 & 1B     & 27.30 \pm 0.16            & 53.90 \pm 0.37                  & 42.70 \pm 0.12  & 59.70 \pm 0.30    \\
      \LLaMmleinVec                 & 7B     & 143.00 \pm 0.22           & 288.00 \pm 0.52                 & 180.00 \pm 0.19 & 304.00 \pm 0.41   \\
      \midrule
      \modernGBERT                  & 134M   & 3.60+-0.29                & 3.70+-0.74                      & 5.42+-0.33      & 4.71+-0.75        \\
      \modernGBERT                  & 1B     & 22.60+-0.40               & 22.50+-0.18                     & 28.70+-0.31     & 26.20+-0.36       \\
      \bottomrule
   \end{tabular}
   \caption{Model Throughput. Numbers are seconds per million tokens. All models were run
      on an RTX A6000 with Bfloat16 data type and with Flash Attention 2, except models with $\dagger$, which did not implement Flash Attention 2.
      Reported uncertainty is the empirical standard deviation on 10 repetitions.}\label{tab:efficiency}
\end{table*}


==> results_table_mteb_full.tex <==
\begin{table*}
   \centering
   \small\begin{tabular}{lllll}
      \toprule
      {Category}         & {Task}                    & {Metric}          & {Reference}                                        \\
      \midrule
      Classification     & AmazonCounterfactual      & Accuracy          & \citet{oneill2021iwishiloved}                      \\
                         & AmazonReviews             & Accuracy          & \citet{keung2020multilingualamazonreviewscorpus}   \\
                         & MTOPDomain                & Accuracy          & \citet{li-etal-2021-mtop}                          \\
                         & MTOPIntent                & Accuracy          & \citet{li-etal-2021-mtop}                          \\
                         & MassiveIntent             & Accuracy          & \citet{fitzgerald-etal-2023-massive}               \\
                         & MassiveScenario           & Accuracy          & \citet{fitzgerald-etal-2023-massive}               \\
      \midrule

      PairClassification & FalseFriendsGermanEnglish & Average Precision & \citet{aari_false_friends}                         \\
                         & PawsXPairClassification   & Average Precision & \citet{yang-etal-2019-paws}                        \\
      \midrule

      Clustering         & BlurbsClusteringP2P       & V-measure         & \citet{wehrli-etal-2023-german}                    \\
                         & BlurbsClusteringS2S       & V-measure         & \citet{wehrli-etal-2023-german}                    \\
                         & TenKGnadClusteringP2P     & V-measure         & \citet{wehrli-etal-2023-german}                    \\
                         & TenKGnadClusteringS2S     & V-measure         & \citet{wehrli-etal-2023-german}                    \\
      \midrule

      Reranking          & MIRACLReranking           & nDCG@10           & \citet{zhang-etal-2023-miracl}                     \\
      \midrule

      Retrieval          & GermanQuAD-Retrieval      & MRR@5             & \citet{moller-etal-2021-germanquad}                \\
                         & GermanDPR                 & DCG@10            & \citet{moller-etal-2021-germanquad}                \\
                         & Xmarket                   & nDCG@10           & \citet{10.1145/3459637.3482493}                    \\
                         & GerDaLIR                  & nDCG@10           & \citet{wrzalik-krechel-2021-gerdalir}              \\
                 %        & LegalQuAD & & \\
      \midrule

      STS                & GermanSTSBenchmark        & Spearman          & \citet{german_sts_benchmark,cer-etal-2017-semeval} \\
                         & STS22                     & Spearman          & \citet{chen-etal-2022-semeval}                     \\

      \bottomrule
   \end{tabular}
   \caption{Overview of tasks included in the German \textit{MTEB(deu,\,v1)} benchmark, grouped by six categories: classification, pairclassification, clustering, reranking, retrieval and STS.}\label{tab:mteb_tasks}
\end{table*}








\begin{table*}
   \centering
   \footnotesize
   \begin{tabular}{lr|cccccc||c}
      \toprule

      Model                                             &
      Params                                            &
      \rotatebox[origin=r]{270}{\makecell[r]{Classification                                                                                                               \\Average}} &
      \rotatebox[origin=r]{270}{\makecell[r]{PairClassification                                                                                                                    \\Average}} &

      \rotatebox[origin=r]{270}{\makecell[r]{Clustering                                                                                                                                \\Average}} &
      \rotatebox[origin=r]{270}{\makecell[r]{Reranking                                                                                                                                 \\Average}} &
      \rotatebox[origin=r]{270}{\makecell[r]{Retrieval                                                                                                                                 \\Average}} &
      \rotatebox[origin=r]{270}{\makecell[r]{STS                                                                                                                                       \\Average}} & Average\\
      \midrule
      \GbertBASE    $^{\phantom{\dagger}}$              & 111M  & 0.634          & 0.504          & 0.274          & 0.118          & 0.226          & 0.402          & 0.360          \\
      \GbertBASE${}^\dagger$                            &       & 0.632          & 0.601          & 0.318          & 0.374          & 0.461          & 0.613          & 0.500          \\[1ex]
      \GbertLARGE$^{\phantom{\dagger}}$                 & 337M  & 0.649          & 0.544          & 0.336          & 0.206          & 0.297          & 0.438          & 0.412          \\

      \GbertLARGE${}^\dagger$                           &       & 0.646          & \textbf{0.662} & 0.334          & 0.389          & 0.493          & 0.603          & 0.521          \\[1ex]


      gerturax-3$^{\phantom{\dagger}}$                  & 135M  & 0.623          & 0.554          & 0.269          & 0.141          & 0.187          & 0.375          & 0.358          \\
      gerturax-3${}^\dagger$                            &       & 0.620          & 0.614          & 0.328          & 0.346          & 0.389          & 0.538          & 0.472          \\[1ex]

      \GebertaBASE$^{\phantom{\dagger}}$                & 139M  & 0.632          & 0.535          & 0.312          & 0.174          & 0.213          & 0.429          & 0.382          \\
      \GebertaBASE${}^\dagger$                          &       & 0.611          & 0.613          & 0.318          & 0.374          & 0.430          & 0.611          & 0.493          \\[1ex]
      \GebertaLARGE                                     & 406M  & 0.642          & 0.533          & 0.287          & 0.223          & 0.274          & 0.424          & 0.397          \\
      \GebertaLARGE${}^\dagger$                         &       & 0.618          & 0.611          & 0.311          & 0.374          & 0.432          & 0.616          & 0.494          \\[1ex]
      \GebertaXLARGE                                    & 887M  & 0.626          & 0.536          & 0.278          & 0.108          & 0.058          & 0.342          & 0.325          \\
      \GebertaXLARGE${}^\dagger$                        &       & 0.638          & 0.631          & 0.323          & 0.414          & 0.462          & 0.655          & 0.521          \\[1ex]
      \XLMRobertaBASE                                   & 279M  & 0.442          & 0.506          & 0.173          & 0.024          & 0.008          & 0.333          & 0.248          \\
      \XLMRobertaBASE${}^\dagger$                       &       & 0.555          & 0.529          & 0.247          & 0.247          & 0.299          & 0.539          & 0.403          \\[1ex]

      \XLMRobertaLARGE                                  & 561M  & 0.510          & 0.510          & 0.172          & 0.048          & 0.026          & 0.320          & 0.264          \\
      \XLMRobertaLARGE${}^\dagger$                      &       & 0.576          & 0.574          & 0.259          & 0.343          & 0.416          & 0.593          & 0.460          \\[1ex]
      \XLMRobertaXLARGE                                 & 3.48B & 0.456          & 0.519          & 0.225          & 0.090          & 0.142          & 0.372          & 0.301          \\
      \XLMRobertaXLARGE${}^\dagger$                     &       & 0.609          & 0.564          & 0.342          & 0.362          & 0.407          & 0.590          & 0.479          \\
      % gerturax-3 & 0.370 & 0.174 & 0.421 & 0.345 & 0.727 & 0.598 & 0.184 & 0.047 & 0.358 \\
      %   jina-embeddings-v3${}^\dagger$ & 0.421 & 0.216 & 0.438 & 0.398 & 0.942 & 0.824 & 0.283 & 0.162 & 0.461 \\
      \midrule
                                      \mmBERTSmall & 142M & & & & & & \\
                                      \mmBERTSmall${}^\dagger$  & 142M & & & & & & \\[1ex]

            \mmBERTBase & 309M & & & & & & \\
                        \mmBERTBase${}^\dagger$  & 309M & & & & & & \\[1ex]

                        \euroBERTsmall & 212M & 0.436& 0.509& 0.240& 0.070 &0.118 & 0.384 & 0.293 \\
                                                \euroBERTsmall${}^\dagger$  & 212M & & & & & & \\[1ex]

                        \euroBERTmid & 609M & & & & & & \\
                                                \euroBERTmid${}^\dagger$  & 609M & & & & & & \\[1ex]

                        \euroBERTlarge & 2.11B & & & & & & \\
                                                \euroBERTlarge${}^\dagger$  & 2.11B & & & & & & \\

      \bottomrule
   \end{tabular}
   \caption{Results on \textit{MTEB(deu,\,v1)} of the German MTEB Benchmark. For each task type, scores were averaged across respective unique tasks.
      We provide results for basis models as well as after supervised training on mMARCO $\dagger$. In all cases, evaluation was done in a zero-shot fashion without further finetuning on the above tasks. Best scores are indicated in bold.
   }
   \label{tab:mteb}
\end{table*}


\begin{table*}
   \centering
   \footnotesize
   \begin{tabular}{lr|cccccc||c}
      \toprule

      Model                                             &
      Params                                            &
      \rotatebox[origin=r]{270}{\makecell[r]{Classification                                                                                                               \\Average}} &
      \rotatebox[origin=r]{270}{\makecell[r]{PairClassification                                                                                                                   \\Average}} &

      \rotatebox[origin=r]{270}{\makecell[r]{Clustering                                                                                                                                \\Average}} &
      \rotatebox[origin=r]{270}{\makecell[r]{Reranking                                                                                                                                 \\Average}} &
      \rotatebox[origin=r]{270}{\makecell[r]{Retrieval                                                                                                                                 \\Average}} &
      \rotatebox[origin=r]{270}{\makecell[r]{STS                                                                                                                                       \\Average}} & Average\\
      \midrule
      %    Llama2Vec 3.2$^{\phantom{\dagger}}$               & 1B    & 0.613          & 0.491          & 0.254          & 0.189          & 0.352          & 0.555          & 0.409          \\

      %   Llama2Vec 3.2${}^\dagger$                         &       & 0.656          & 0.570          & 0.311          & 0.450          & 0.476          & 0.646          & 0.518          \\[1ex]
      %   Llama2Vec 3.1$^{\phantom{\dagger}}$               & 8B    & 0.688          & 0.524          & 0.315          & 0.339          & 0.410          & 0.605          & 0.480          \\

      %      Llama2Vec 3.1${}^\dagger$                         &       & 0.683          & 0.598          & 0.327          & 0.477          & 0.509          & 0.688          & 0.547          \\
      % \midrule
      \LLaMmleinVec$^{\phantom{\dagger}}$ (ext1)        & 120M  & 0.546          & 0.529          & 0.261          & 0.139          & 0.224          & 0.188          & 0.315          \\
      \LLaMmleinVec${}^\dagger$  (ext1)                 & 120M  & 0.599          & 0.575          & 0.308          & 0.325          & 0.425          & 0.592          & 0.471          \\[1ex]
      \LLaMmleinVec$^{\phantom{\dagger}}$ (ext2)        & 120M  & 0.457          & 0.525          & 0.202          & 0.118          & 0.117          & 0.205          & 0.271          \\
      \LLaMmleinVec${}^\dagger$  (ext2)                 & 120M  & 0.607          & 0.588          & 0.295          & 0.305          & 0.339          & 0.498          & 0.439          \\[1ex]
      \LLaMmleinVec$^{\phantom{\dagger}}$ (ext1+2)      & 120M  & 0.339          & 0.530          & 0.098          & 0.046          & 0.009          & 0.107          & 0.188          \\
      \LLaMmleinVec${}^\dagger$  (ext1+2)               & 120M  & 0.517          & 0.563          & 0.263          & 0.251          & 0.355          & 0.554          & 0.417          \\


      % LLäMmlein2Vec$^{\phantom{\dagger}}$              & 120M  & 0.470          & 0.517          & 0.275          & 0.134          & 0.128          & 0.455          & 0.330          \\
      \midrule
      \LLaMmleinVec$^{\phantom{\dagger}}$ (ext1)        & 1B    & 0.641          & 0.542          & 0.308          & 0.183          & 0.276          & 0.442          & 0.399          \\
      \LLaMmleinVec${}^\dagger$  (ext1)                 & 1B    & 0.670          & 0.625          & \textbf{0.343} & 0.433          & 0.511          & 0.660          & 0.540          \\[1ex]
      \LLaMmleinVec$^{\phantom{\dagger}}$ (ext2)        & 1B    & 0.617          & 0.541          & 0.299          & 0.189          & 0.280          & 0.431          & 0.393          \\
      \LLaMmleinVec${}^\dagger$  (ext2)                 & 1B    & 0.666          & 0.622          & 0.330          & 0.433          & 0.499          & 0.644          & 0.532          \\[1ex]
      \LLaMmleinVec$^{\phantom{\dagger}}$ (ext1+2)      & 1B    & 0.337          & 0.538          & 0.075          & 0.062          & 0.010          & 0.217          & 0.206          \\
      \LLaMmleinVec${}^\dagger$  (ext1+2)               & 1B    & 0.647          & 0.611          & 0.325          & 0.421          & 0.481          & 0.640          & 0.521          \\


      %LLäMmlein2Vec${}^\dagger$                         &       & 0.593          & 0.586          & 0.307          & 0.349          & 0.423          & 0.612          & 0.478          \\[1ex]
      %LLäMmlein2Vec$^{\phantom{\dagger}}$               & 1B    & \textbf{0.695} & 0.577          & 0.345          & 0.314          & 0.416          & 0.566          & 0.486          \\

      %LLäMmlein2Vec${}^\dagger$                         &       & 0.674          & 0.624          & 0.344          & 0.451          & 0.505          & 0.658          & 0.543          \\[1ex]
      %    LLäMmlein2Vec$^{\phantom{\dagger}}$               & 7B    & 0.713          & 0.580          & 0.342          & 0.322          & 0.443          & 0.603          & 0.501          \\

      %  LLäMmlein2Vec${}^\dagger$                         &       & 0.688          & 0.631          & \textbf{0.349} & \textbf{0.483} & \textbf{0.523} & \textbf{0.694} & \textbf{0.561} \\
      \midrule
      \LLaMmleinVec$^{\phantom{\dagger}}$ (ext1)        & 7B    & 0.683          & 0.558          & 0.249          & 0.169          & 0.266          & 0.333          & 0.376          \\
      \LLaMmleinVec${}^\dagger$  (ext1)                 & 7B    & \textbf{0.687} & 0.636          & 0.339          & \textbf{0.477} & \textbf{0.522} & \textbf{0.682} & \textbf{0.557} \\[1ex]
      \LLaMmleinVec$^{\phantom{\dagger}}$ (ext2)        & 7B    & 0.679          & 0.555          & 0.323          & 0.187          & 0.309          & 0.462          & 0.419          \\
      \LLaMmleinVec${}^\dagger$  (ext2)                 & 7B    & 0.683          & 0.628          & 0.337          & 0.471          & 0.517          & 0.680          & 0.553          \\[1ex]
      \LLaMmleinVec$^{\phantom{\dagger}}$ (ext1+2)      & 7B    & 0.349          & 0.525          & 0.072          & 0.047          & 0.005          & 0.182          & 0.197          \\
      \LLaMmleinVec${}^\dagger$  (ext1+2)               & 7B    & 0.677          & 0.615          & 0.327          & 0.460          & 0.506          & 0.663          & 0.541          \\


      \midrule
      \modernGBERT $^{\phantom{\dagger}}$               & 134M  & 0.639          & 0.537          & 0.293          & 0.139          & 0.241          & 0.449          & 0.383          \\

      \modernGBERT ${}^\dagger$                         &       & 0.602          & 0.606          & 0.303          & 0.364          & 0.432          & 0.602          & 0.485          \\[1ex]



      \modernGBERT $^{\phantom{\dagger}}$      + ext1+2 & 134M  & 0.642          & 0.536          & 0.296          & 0.120          & 0.213          & 0.445          & 0.376          \\

      \modernGBERT ${}^\dagger$    + ext1+2             &       & 0.629          & 0.612          & 0.312          & 0.404          & 0.446          & 0.606          & 0.501          \\
      \midrule

      \modernGBERT $^{\phantom{\dagger}}$               & 1B    & 0.665          & 0.544          & 0.318          & 0.097          & 0.199          & 0.418          & 0.374          \\

      \modernGBERT ${}^\dagger$                         &       & 0.659          & 0.641          & 0.339          & 0.463          & 0. 511         & 0.681          & 0.549          \\[1ex]



      \modernGBERT $^{\phantom{\dagger}}$   + ext1+2    & 1B    & 0.659          & 0.540          & 0.307          & 0.088          & 0.191          & 0.410          & 0.366          \\


      \modernGBERT${}^\dagger$     + ext1+2             &       & 0.659          & 0.654          & 0.338          & 0.459          & 0.513          & \textbf{0.682} & 0.551          \\
      \bottomrule
   \end{tabular}
   \caption{Results on \textit{MTEB(deu,\,v1)} of the German MTEB Benchmark. For each task type, scores were averaged across respective unique tasks.
      We provide results for basis models as well as after supervised training on mMARCO $\dagger$. In all cases, evaluation was done in a zero-shot fashion without further finetuning on the above tasks. Best scores are indicated in bold.
   }
   \label{tab:mteb}
\end{table*}


==> table_architecture.tex <==
\begin{table*}[!t]
    \small
    \centering
    \begin{tabular}{lccccc}
        \toprule
                               & \multicolumn{2}{c}{\modernGBERT} & \multicolumn{3}{c}{\clap{LLäMmlein2Vec}}                                              \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-6}
        Parameters             & 134M                             & 1B                                       & 120M         & 1B           & 7B           \\
        \midrule
        Vocabulary             & \num{31168}                      & \num{31168}                              & \num{32064}  & \num{32064}  & \num{32064}  \\
        Unused Tokens          & 66                               & 66                                       & 54           & 54           & 54           \\
        Layers                 & 22                               & 28                                       & 12           & 22           & 32           \\
        Hidden Size            & \num{768}                        & \num{2048}                               & \num{768}    & \num{2048}   & \num{4096}   \\
        Transformer Block      & Pre-Norm                         & Pre-Norm                                 & Post-Norm    & Post-Norm    & Post-Norm    \\
        Activation Function    & GeLU                             & GeLU                                     & SiLU         & SiLU         & SiLU         \\
        %Linear Bias & False & False & False & False & False\\
        %Attention & Multi-head & Multi-head \\
        Attention Heads        & 12                               & 32                                       & 12           & 32           & 32           \\
        Head Size              & 64                               & 64                                       & 64           & 64           & 128          \\
        Intermediate Size      & \num{1152}                       & \num{3072}                               & \num{2048}   & \num{5632}   & \num{11008}  \\
        %GLU Expansion & 2304 & 6142 & --- & --- & --- \\
        Normalization          & LayerNorm                        & LayerNorm                                & RMSNorm      & RMSNorm      & RMSNorm      \\
        Norm Epsilon           & \num{1e-5}                       & \num{1e-5}                               & \num{1e-5}   & \num{1e-5}   & \num{1e-5}   \\
        %Norm Bias & False & False & False \\
        RoPE theta             & \num{160000}                     & \num{160000}                             & \num{160000} & \num{160000} & \num{160000} \\
        Global Attention       & Every three layers               & Every three layers                       & Every layer  & Every layer  & Every layer  \\
        Local Attention Window & 128                              & 128                                      & ---          & ---          & ---          \\
        Local Attn RoPE theta  & \num{10000}                      & \num{10000}                              & ---          & ---          & ---          \\
        \bottomrule
    \end{tabular}
    \caption{Model design of the \modernGBERT and LLäMmlein2Vec model family.}
    \label{tab:architecture}
\end{table*}

